Immersed boundary-finite element model of fluid-structure interaction in the aortic root

It has long been recognized that aortic root elasticity helps to ensure efficient aortic valve closure, but our understanding of the functional importance of the elasticity and geometry of the aortic root continues to evolve as increasingly detailed in vivo imaging data become available. Herein, we describe fluid-structure interaction models of the aortic root, including the aortic valve leaflets, the sinuses of Valsalva, the aortic annulus, and the sinotubular junction, that employ a version of Peskin's immersed boundary (IB) method with a finite element (FE) description of the structural elasticity. We develop both an idealized model of the root with three-fold symmetry of the aortic sinuses and valve leaflets, and a more realistic model that accounts for the differences in the sizes of the left, right, and noncoronary sinuses and corresponding valve cusps. As in earlier work, we use fiber-based models of the valve leaflets, but this study extends earlier IB models of the aortic root by employing incompressible hyperelastic models of the mechanics of the sinuses and ascending aorta using a constitutive law fit to experimental data from human aortic root tissue. In vivo pressure loading is accounted for by a backwards displacement method that determines the unloaded configurations of the root models. Our models yield realistic cardiac output at physiological pressures, with low transvalvular pressure differences during forward flow, minimal regurgitation during valve closure, and realistic pressure loads when the valve is closed during diastole. Further, results from high-resolution computations demonstrate that IB models of the aortic valve are able to produce essentially grid-converged dynamics at practical grid spacings for the high-Reynolds number flows of the aortic root.

==> images/Commissura_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Commissura_sp!}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 06:51:34
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Max Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{60}%
\psfrag{v02}[r][r]{70}%
\psfrag{v03}[r][r]{80}%
\psfrag{v04}[r][r]{90}%
\psfrag{v05}[r][r]{100}%
\psfrag{v06}[r][r]{110}%
\psfrag{v07}[r][r]{120}%
\psfrag{v08}[r][r]{130}%
\psfrag{v09}[r][r]{140}%
\psfrag{v10}[r][r]{150}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{Commissura_sp1.eps}}%
\end{psfrags}%
%
% End Commissura_sp!.tex


==> images/Convergence_plot.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Convergence_plot}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           23-Oct-2013 09:27:43
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Residuals (mm)\end{tabular}}%
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Iteration Number\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{Convergence_plot.eps}}%
\end{psfrags}%
%
% End Convergence_plot.tex


==> images/Figure_6_new.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Figure_6_new}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           06-Aug-2013 13:07:17
% eps bounding box:     15 cm x 8.3021 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s28}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Gap = 0.4375\\\end{tabular}}%
\psfrag{s29}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Bnd = 0.125\end{tabular}}%
\psfrag{s30}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Bnd = 0.15\end{tabular}}%
\psfrag{s31}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Bnd = 0.175\end{tabular}}%
\psfrag{s32}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Gap = 0.5\\ \\Pressure (mmHg)\end{tabular}}%
\psfrag{s33}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Gap = 0.625\\ \end{tabular}}%
\psfrag{s34}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s) \\ \\ \end{tabular}}%
\psfrag{s35}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s) \\ \\ \end{tabular}}%
\psfrag{s36}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s) \\ \\ \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{3}%
\psfrag{x05}[t][t]{4}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{2}%
\psfrag{x09}[t][t]{3}%
\psfrag{x10}[t][t]{4}%
\psfrag{x11}[t][t]{0}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{2}%
\psfrag{x14}[t][t]{3}%
\psfrag{x15}[t][t]{4}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{1}%
\psfrag{x18}[t][t]{2}%
\psfrag{x19}[t][t]{3}%
\psfrag{x20}[t][t]{4}%
\psfrag{x21}[t][t]{0}%
\psfrag{x22}[t][t]{1}%
\psfrag{x23}[t][t]{2}%
\psfrag{x24}[t][t]{3}%
\psfrag{x25}[t][t]{4}%
\psfrag{x26}[t][t]{0}%
\psfrag{x27}[t][t]{1}%
\psfrag{x28}[t][t]{2}%
\psfrag{x29}[t][t]{3}%
\psfrag{x30}[t][t]{4}%
\psfrag{x31}[t][t]{0}%
\psfrag{x32}[t][t]{1}%
\psfrag{x33}[t][t]{2}%
\psfrag{x34}[t][t]{3}%
\psfrag{x35}[t][t]{4}%
\psfrag{x36}[t][t]{0}%
\psfrag{x37}[t][t]{1}%
\psfrag{x38}[t][t]{2}%
\psfrag{x39}[t][t]{3}%
\psfrag{x40}[t][t]{4}%
\psfrag{x41}[t][t]{0}%
\psfrag{x42}[t][t]{1}%
\psfrag{x43}[t][t]{2}%
\psfrag{x44}[t][t]{3}%
\psfrag{x45}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{ }%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{ }%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{120}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{ }%
\psfrag{v10}[r][r]{ }%
\psfrag{v11}[r][r]{60}%
\psfrag{v12}[r][r]{ }%
\psfrag{v13}[r][r]{ }%
\psfrag{v14}[r][r]{120}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{ }%
\psfrag{v17}[r][r]{ }%
\psfrag{v18}[r][r]{60}%
\psfrag{v19}[r][r]{ }%
\psfrag{v20}[r][r]{ }%
\psfrag{v21}[r][r]{120}%
\psfrag{v22}[r][r]{0}%
\psfrag{v23}[r][r]{ }%
\psfrag{v24}[r][r]{ }%
\psfrag{v25}[r][r]{60}%
\psfrag{v26}[r][r]{ }%
\psfrag{v27}[r][r]{ }%
\psfrag{v28}[r][r]{120}%
\psfrag{v29}[r][r]{0}%
\psfrag{v30}[r][r]{ }%
\psfrag{v31}[r][r]{ }%
\psfrag{v32}[r][r]{60}%
\psfrag{v33}[r][r]{ }%
\psfrag{v34}[r][r]{ }%
\psfrag{v35}[r][r]{120}%
\psfrag{v36}[r][r]{0}%
\psfrag{v37}[r][r]{ }%
\psfrag{v38}[r][r]{ }%
\psfrag{v39}[r][r]{60}%
\psfrag{v40}[r][r]{ }%
\psfrag{v41}[r][r]{ }%
\psfrag{v42}[r][r]{120}%
\psfrag{v43}[r][r]{0}%
\psfrag{v44}[r][r]{ }%
\psfrag{v45}[r][r]{ }%
\psfrag{v46}[r][r]{60}%
\psfrag{v47}[r][r]{ }%
\psfrag{v48}[r][r]{ }%
\psfrag{v49}[r][r]{120}%
\psfrag{v50}[r][r]{0}%
\psfrag{v51}[r][r]{ }%
\psfrag{v52}[r][r]{ }%
\psfrag{v53}[r][r]{60}%
\psfrag{v54}[r][r]{ }%
\psfrag{v55}[r][r]{ }%
\psfrag{v56}[r][r]{120}%
\psfrag{v57}[r][r]{0}%
\psfrag{v58}[r][r]{ }%
\psfrag{v59}[r][r]{ }%
\psfrag{v60}[r][r]{60}%
\psfrag{v61}[r][r]{ }%
\psfrag{v62}[r][r]{ }%
\psfrag{v63}[r][r]{120}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{Figure_6_new.eps}}%
\end{psfrags}%
%
% End Figure_6_new.tex


==> images/Residuals-1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{Residuals}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           17-Jun-2014 08:38:04
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Residual (m)\end{tabular}}%
\psfrag{s06}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Iteration Number\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Asymmetric Model}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Symmetric Model}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Asymmetric Model}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
\psfrag{ypower2}[Bl][Bl]{$\times 10^{-3}$}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{Residuals.eps}}%
\end{psfrags}%
%
% End Residuals.tex


==> images/SJT_closed.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{SJT_closed}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 09:17:09
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Time (s)\end{tabular}}%
\psfrag{s03}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Displacement (cm)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{\Large 1}%
\psfrag{x02}[t][t]{ }%
\psfrag{x03}[t][t]{\Large 2}%
\psfrag{x04}[t][t]{ }%
\psfrag{x05}[t][t]{\Large 3}%
\psfrag{x06}[t][t]{ }%
\psfrag{x07}[t][t]{\Large 4}%
%
% yticklabels:
\psfrag{v01}[r][r]{\Large 0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{ }%
\psfrag{v04}[r][r]{ }%
\psfrag{v05}[r][r]{\Large 0.2}%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{ }%
\psfrag{v08}[r][r]{ }%
\psfrag{v09}[r][r]{\Large 0.4}%
\psfrag{v10}[r][r]{ }%
\psfrag{v11}[r][r]{ }%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{SJT_closed.eps}}%
\end{psfrags}%
%
% End SJT_closed.tex


==> images/SJT_open.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{SJT_open}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 09:16:06
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Time (s)\end{tabular}}%
\psfrag{s03}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Displacement (cm)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{\Large 1}%
\psfrag{x02}[t][t]{ }%
\psfrag{x03}[t][t]{\Large 2}%
\psfrag{x04}[t][t]{ }%
\psfrag{x05}[t][t]{\Large 3}%
\psfrag{x06}[t][t]{ }%
\psfrag{x07}[t][t]{\Large 4}%
%
% yticklabels:
\psfrag{v01}[r][r]{\Large 0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{ }%
\psfrag{v04}[r][r]{ }%
\psfrag{v05}[r][r]{\Large 0.02}%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{ }%
\psfrag{v08}[r][r]{ }%
\psfrag{v09}[r][r]{\Large 0.04}%
\psfrag{v10}[r][r]{ }%
\psfrag{v11}[r][r]{ }%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{SJT_open.eps}}%
\end{psfrags}%
%
% End SJT_open.tex


==> images/SJT_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{SJT_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 06:51:58
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Max Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{80}%
\psfrag{v02}[r][r]{100}%
\psfrag{v03}[r][r]{120}%
\psfrag{v04}[r][r]{140}%
\psfrag{v05}[r][r]{160}%
\psfrag{v06}[r][r]{180}%
\psfrag{v07}[r][r]{200}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{SJT_sp1.eps}}%
\end{psfrags}%
%
% End SJT_sp1.tex


==> images/STJ_asym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{STJ_asym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:40:43
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Right}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Left}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Non-Coronary}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Right}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.3}%
\psfrag{v02}[r][r]{-0.2}%
\psfrag{v03}[r][r]{-0.1}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{0.1}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.3}%
\psfrag{v08}[r][r]{0.4}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{STJ_asym_dx.eps}}%
\end{psfrags}%
%
% End STJ_asym_dx.tex


==> images/STJ_asym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{STJ_asym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 09:27:49
% eps bounding box:     15 cm x 11.2232 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{STJ_asym_dx_2.eps}}%
\end{psfrags}%
%
% End STJ_asym_dx_2.tex


==> images/STJ_sym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{STJ_sym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:30:52
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.4}%
\psfrag{v02}[r][r]{-0.3}%
\psfrag{v03}[r][r]{-0.2}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.1}%
\psfrag{v07}[r][r]{0.2}%
\psfrag{v08}[r][r]{0.3}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{STJ_sym_dx.eps}}%
\end{psfrags}%
%
% End STJ_sym_dx.tex


==> images/STJ_sym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{STJ_sym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 10:05:33
% eps bounding box:     15 cm x 10.6607 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{STJ_sym_dx_2.eps}}%
\end{psfrags}%
%
% End STJ_sym_dx_2.tex


==> images/STJ_sym_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{STJ_sym_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:08:06
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}First Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{90}%
\psfrag{v02}[r][r]{100}%
\psfrag{v03}[r][r]{110}%
\psfrag{v04}[r][r]{120}%
\psfrag{v05}[r][r]{130}%
\psfrag{v06}[r][r]{140}%
\psfrag{v07}[r][r]{150}%
\psfrag{v08}[r][r]{160}%
\psfrag{v09}[r][r]{170}%
\psfrag{v10}[r][r]{180}%
\psfrag{v11}[r][r]{190}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{STJ_sym_sp1.eps}}%
\end{psfrags}%
%
% End STJ_sym_sp1.tex


==> images/aorta_asym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aorta_asym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:40:07
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Right}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Left}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Non-Coronary}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Right}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.3}%
\psfrag{v02}[r][r]{-0.2}%
\psfrag{v03}[r][r]{-0.1}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{0.1}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.3}%
\psfrag{v08}[r][r]{0.4}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_asym_dx.eps}}%
\end{psfrags}%
%
% End aorta_asym_dx.tex


==> images/aorta_asym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aorta_asym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 09:24:39
% eps bounding box:     15 cm x 11.2232 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
\psfrag{v09}[r][r]{0.7}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_asym_dx_2.eps}}%
\end{psfrags}%
%
% End aorta_asym_dx_2.tex


==> images/aorta_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aosrta_sp!}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 06:51:09
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Max Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{60}%
\psfrag{v02}[r][r]{70}%
\psfrag{v03}[r][r]{80}%
\psfrag{v04}[r][r]{90}%
\psfrag{v05}[r][r]{100}%
\psfrag{v06}[r][r]{110}%
\psfrag{v07}[r][r]{120}%
\psfrag{v08}[r][r]{130}%
\psfrag{v09}[r][r]{140}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_sp1.eps}}%
\end{psfrags}%
%
% End aosrta_sp!.tex


==> images/aorta_sym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aorta_sym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:32:06
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.4}%
\psfrag{v02}[r][r]{-0.3}%
\psfrag{v03}[r][r]{-0.2}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.1}%
\psfrag{v07}[r][r]{0.2}%
\psfrag{v08}[r][r]{0.3}%
\psfrag{v09}[r][r]{0.4}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_sym_dx.eps}}%
\end{psfrags}%
%
% End aorta_sym_dx.tex


==> images/aorta_sym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aorta_sym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 10:06:43
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_sym_dx_2.eps}}%
\end{psfrags}%
%
% End aorta_sym_dx_2.tex


==> images/aorta_sym_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{aorta_sym_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:07:43
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}First Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{60}%
\psfrag{v02}[r][r]{70}%
\psfrag{v03}[r][r]{80}%
\psfrag{v04}[r][r]{90}%
\psfrag{v05}[r][r]{100}%
\psfrag{v06}[r][r]{110}%
\psfrag{v07}[r][r]{120}%
\psfrag{v08}[r][r]{130}%
\psfrag{v09}[r][r]{140}%
\psfrag{v10}[r][r]{150}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{aorta_sym_sp1.eps}}%
\end{psfrags}%
%
% End aorta_sym_sp1.tex


==> images/asym_flow-1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:19:37
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{flow_asym.eps}}%
\end{psfrags}%
%
% End flow_asym.tex


==> images/asym_flow.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:19:37
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{flow_asym.eps}}%
\end{psfrags}%
%
% End flow_asym.tex


==> images/asym_pressure-1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{pres_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:19:57
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Pressure (mmHg)\end{tabular}}%
\psfrag{s06}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Aorta}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{40}%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{80}%
\psfrag{v06}[r][r]{100}%
\psfrag{v07}[r][r]{120}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{pres_asym.eps}}%
\end{psfrags}%
%
% End pres_asym.tex


==> images/asym_pressure.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{pres_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:19:57
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Pressure (mmHg)\end{tabular}}%
\psfrag{s06}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Aorta}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{40}%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{80}%
\psfrag{v06}[r][r]{100}%
\psfrag{v07}[r][r]{120}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{pres_asym.eps}}%
\end{psfrags}%
%
% End pres_asym.tex


==> images/commis_asym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commis_asym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:40:24
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Right}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Left}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Non-Coronary}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Right}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.4}%
\psfrag{v02}[r][r]{-0.3}%
\psfrag{v03}[r][r]{-0.2}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.1}%
\psfrag{v07}[r][r]{0.2}%
\psfrag{v08}[r][r]{0.3}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commis_asym_dx.eps}}%
\end{psfrags}%
%
% End commis_asym_dx.tex


==> images/commis_asym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commis_asym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 09:27:26
% eps bounding box:     15 cm x 11.2232 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commis_asym_dx_2.eps}}%
\end{psfrags}%
%
% End commis_asym_dx_2.tex


==> images/commis_sym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commis_sym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:31:26
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.4}%
\psfrag{v02}[r][r]{-0.3}%
\psfrag{v03}[r][r]{-0.2}%
\psfrag{v04}[r][r]{-0.1}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.1}%
\psfrag{v07}[r][r]{0.2}%
\psfrag{v08}[r][r]{0.3}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commis_sym_dx.eps}}%
\end{psfrags}%
%
% End commis_sym_dx.tex


==> images/commis_sym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commis_sym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 10:05:59
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.1}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.3}%
\psfrag{v06}[r][r]{0.4}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commis_sym_dx_2.eps}}%
\end{psfrags}%
%
% End commis_sym_dx_2.tex


==> images/commiss_asym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commiss_asym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 06:58:36
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}First Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Right}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Left}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Non-Coronary}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Right}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.03}%
\psfrag{v02}[r][r]{-0.02}%
\psfrag{v03}[r][r]{-0.01}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{0.01}%
\psfrag{v06}[r][r]{0.02}%
\psfrag{v07}[r][r]{0.03}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commiss_asym_dx.eps}}%
\end{psfrags}%
%
% End commiss_asym_dx.tex


==> images/commiss_sym_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{commiss_sym_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:09:30
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}First Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{60}%
\psfrag{v02}[r][r]{80}%
\psfrag{v03}[r][r]{100}%
\psfrag{v04}[r][r]{120}%
\psfrag{v05}[r][r]{140}%
\psfrag{v06}[r][r]{160}%
\psfrag{v07}[r][r]{180}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{commiss_sym_sp1.eps}}%
\end{psfrags}%
%
% End commiss_sym_sp1.tex


==> images/convergence_sym_asym.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{convergence_sym_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-May-2014 15:53:21
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Iteration Number\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Residual (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0} Symmetric Model}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0} Asymmetric Model}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
\psfrag{ypower2}[Bl][Bl]{ }%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{convergence_sym_asym.eps}}%
\end{psfrags}%
%
% End convergence_sym_asym.tex


==> images/fig_Flow.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_Flow}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9. 4)
% created on:           07-Aug-2013 20:15:54
% eps bounding box:     15 cm x 8.3021 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s28}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Reference\\distance \\  \\  \\\end{tabular}}%
\psfrag{s29}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} 85\% $c_{b}$\end{tabular}}%
\psfrag{s30}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$c_{b}$\end{tabular}}%
\psfrag{s31}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}115\% $c_{b}$\end{tabular}}%
\psfrag{s32}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Distance\\15\% increase \\ \\Flow (ml/s)\end{tabular}}%
\psfrag{s33}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Distance\\40\% increase\\  \\  \\\end{tabular}}%
\psfrag{s34}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}  \end{tabular}}%
\psfrag{s35}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s) \end{tabular}}%
\psfrag{s36}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}  \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{3}%
\psfrag{x05}[t][t]{4}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{2}%
\psfrag{x09}[t][t]{3}%
\psfrag{x10}[t][t]{4}%
\psfrag{x11}[t][t]{0}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{2}%
\psfrag{x14}[t][t]{3}%
\psfrag{x15}[t][t]{4}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{1}%
\psfrag{x18}[t][t]{2}%
\psfrag{x19}[t][t]{3}%
\psfrag{x20}[t][t]{4}%
\psfrag{x21}[t][t]{0}%
\psfrag{x22}[t][t]{1}%
\psfrag{x23}[t][t]{2}%
\psfrag{x24}[t][t]{3}%
\psfrag{x25}[t][t]{4}%
\psfrag{x26}[t][t]{0}%
\psfrag{x27}[t][t]{1}%
\psfrag{x28}[t][t]{2}%
\psfrag{x29}[t][t]{3}%
\psfrag{x30}[t][t]{4}%
\psfrag{x31}[t][t]{0}%
\psfrag{x32}[t][t]{1}%
\psfrag{x33}[t][t]{2}%
\psfrag{x34}[t][t]{3}%
\psfrag{x35}[t][t]{4}%
\psfrag{x36}[t][t]{0}%
\psfrag{x37}[t][t]{1}%
\psfrag{x38}[t][t]{2}%
\psfrag{x39}[t][t]{3}%
\psfrag{x40}[t][t]{4}%
\psfrag{x41}[t][t]{0}%
\psfrag{x42}[t][t]{1}%
\psfrag{x43}[t][t]{2}%
\psfrag{x44}[t][t]{3}%
\psfrag{x45}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-400}%
\psfrag{v02}[r][r]{- }%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{ }%
\psfrag{v05}[r][r]{400}%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{800}%
\psfrag{v08}[r][r]{-400}%
\psfrag{v09}[r][r]{ }%
\psfrag{v10}[r][r]{0}%
\psfrag{v11}[r][r]{ }%
\psfrag{v12}[r][r]{400}%
\psfrag{v13}[r][r]{ }%
\psfrag{v14}[r][r]{800}%
\psfrag{v15}[r][r]{-400}%
\psfrag{v16}[r][r]{ }%
\psfrag{v17}[r][r]{0}%
\psfrag{v18}[r][r]{ }%
\psfrag{v19}[r][r]{400}%
\psfrag{v20}[r][r]{ }%
\psfrag{v21}[r][r]{800}%
\psfrag{v22}[r][r]{-400}%
\psfrag{v23}[r][r]{ }%
\psfrag{v24}[r][r]{0}%
\psfrag{v25}[r][r]{ }%
\psfrag{v26}[r][r]{400}%
\psfrag{v27}[r][r]{ }%
\psfrag{v28}[r][r]{800}%
\psfrag{v29}[r][r]{-400}%
\psfrag{v30}[r][r]{ }%
\psfrag{v31}[r][r]{0}%
\psfrag{v32}[r][r]{ }%
\psfrag{v33}[r][r]{400}%
\psfrag{v34}[r][r]{ }%
\psfrag{v35}[r][r]{800}%
\psfrag{v36}[r][r]{-400}%
\psfrag{v37}[r][r]{ }%
\psfrag{v38}[r][r]{0}%
\psfrag{v39}[r][r]{ }%
\psfrag{v40}[r][r]{400}%
\psfrag{v41}[r][r]{ }%
\psfrag{v42}[r][r]{800}%
\psfrag{v43}[r][r]{-400}%
\psfrag{v44}[r][r]{ }%
\psfrag{v45}[r][r]{0}%
\psfrag{v46}[r][r]{ }%
\psfrag{v47}[r][r]{400}%
\psfrag{v48}[r][r]{ }%
\psfrag{v49}[r][r]{800}%
\psfrag{v50}[r][r]{-400}%
\psfrag{v51}[r][r]{ }%
\psfrag{v52}[r][r]{0}%
\psfrag{v53}[r][r]{ }%
\psfrag{v54}[r][r]{400}%
\psfrag{v55}[r][r]{ }%
\psfrag{v56}[r][r]{800}%
\psfrag{v57}[r][r]{-400}%
\psfrag{v58}[r][r]{ }%
\psfrag{v59}[r][r]{0}%
\psfrag{v60}[r][r]{ }%
\psfrag{v61}[r][r]{400}%
\psfrag{v62}[r][r]{ }%
\psfrag{v63}[r][r]{800}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{fig_Flow.eps}}%
\end{psfrags}%
%
% End fig_Flow.tex


==> images/fig_P.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_P}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Aug-2013 20:15:27
% eps bounding box:     15 cm x 8.3021 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s28}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Reference\\distance \\  \\  \\\end{tabular}}%
\psfrag{s29}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} 85\% $c_{b}$\end{tabular}}%
\psfrag{s30}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$c_{b}$\end{tabular}}%
\psfrag{s31}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}115\% $c_{b}$\end{tabular}}%
\psfrag{s32}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Distance\\15\% increase \\ \\Pressure (mmHg)\end{tabular}}%
\psfrag{s33}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Distance\\40\% increase\\  \\  \\\end{tabular}}%
\psfrag{s34}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}  \end{tabular}}%
\psfrag{s35}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s) \end{tabular}}%
\psfrag{s36}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}  \end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{3}%
\psfrag{x05}[t][t]{4}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{2}%
\psfrag{x09}[t][t]{3}%
\psfrag{x10}[t][t]{4}%
\psfrag{x11}[t][t]{0}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{2}%
\psfrag{x14}[t][t]{3}%
\psfrag{x15}[t][t]{4}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{1}%
\psfrag{x18}[t][t]{2}%
\psfrag{x19}[t][t]{3}%
\psfrag{x20}[t][t]{4}%
\psfrag{x21}[t][t]{0}%
\psfrag{x22}[t][t]{1}%
\psfrag{x23}[t][t]{2}%
\psfrag{x24}[t][t]{3}%
\psfrag{x25}[t][t]{4}%
\psfrag{x26}[t][t]{0}%
\psfrag{x27}[t][t]{1}%
\psfrag{x28}[t][t]{2}%
\psfrag{x29}[t][t]{3}%
\psfrag{x30}[t][t]{4}%
\psfrag{x31}[t][t]{0}%
\psfrag{x32}[t][t]{1}%
\psfrag{x33}[t][t]{2}%
\psfrag{x34}[t][t]{3}%
\psfrag{x35}[t][t]{4}%
\psfrag{x36}[t][t]{0}%
\psfrag{x37}[t][t]{1}%
\psfrag{x38}[t][t]{2}%
\psfrag{x39}[t][t]{3}%
\psfrag{x40}[t][t]{4}%
\psfrag{x41}[t][t]{0}%
\psfrag{x42}[t][t]{1}%
\psfrag{x43}[t][t]{2}%
\psfrag{x44}[t][t]{3}%
\psfrag{x45}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{ }%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{ }%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{120}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{ }%
\psfrag{v10}[r][r]{ }%
\psfrag{v11}[r][r]{60}%
\psfrag{v12}[r][r]{ }%
\psfrag{v13}[r][r]{ }%
\psfrag{v14}[r][r]{120}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{ }%
\psfrag{v17}[r][r]{ }%
\psfrag{v18}[r][r]{60}%
\psfrag{v19}[r][r]{ }%
\psfrag{v20}[r][r]{ }%
\psfrag{v21}[r][r]{120}%
\psfrag{v22}[r][r]{0}%
\psfrag{v23}[r][r]{ }%
\psfrag{v24}[r][r]{ }%
\psfrag{v25}[r][r]{60}%
\psfrag{v26}[r][r]{ }%
\psfrag{v27}[r][r]{ }%
\psfrag{v28}[r][r]{120}%
\psfrag{v29}[r][r]{0}%
\psfrag{v30}[r][r]{ }%
\psfrag{v31}[r][r]{ }%
\psfrag{v32}[r][r]{60}%
\psfrag{v33}[r][r]{ }%
\psfrag{v34}[r][r]{ }%
\psfrag{v35}[r][r]{120}%
\psfrag{v36}[r][r]{0}%
\psfrag{v37}[r][r]{ }%
\psfrag{v38}[r][r]{ }%
\psfrag{v39}[r][r]{60}%
\psfrag{v40}[r][r]{ }%
\psfrag{v41}[r][r]{ }%
\psfrag{v42}[r][r]{120}%
\psfrag{v43}[r][r]{0}%
\psfrag{v44}[r][r]{ }%
\psfrag{v45}[r][r]{ }%
\psfrag{v46}[r][r]{60}%
\psfrag{v47}[r][r]{ }%
\psfrag{v48}[r][r]{ }%
\psfrag{v49}[r][r]{120}%
\psfrag{v50}[r][r]{0}%
\psfrag{v51}[r][r]{ }%
\psfrag{v52}[r][r]{ }%
\psfrag{v53}[r][r]{60}%
\psfrag{v54}[r][r]{ }%
\psfrag{v55}[r][r]{ }%
\psfrag{v56}[r][r]{120}%
\psfrag{v57}[r][r]{0}%
\psfrag{v58}[r][r]{ }%
\psfrag{v59}[r][r]{ }%
\psfrag{v60}[r][r]{60}%
\psfrag{v61}[r][r]{ }%
\psfrag{v62}[r][r]{ }%
\psfrag{v63}[r][r]{120}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{fig_P.eps}}%
\end{psfrags}%
%
% End fig_P.tex


==> images/figure_3.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{figure_3}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           26-Jul-2013 18:22:04
% eps bounding box:     15 cm x 11.25 cm
% comment:
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}residual (m)\end{tabular}}%
\psfrag{s07}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}iteration number\end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}change relative to mean radius (\%)\end{tabular}}%
\psfrag{s18}[l][l]{\color[rgb]{0,0,0}change relative to mean radius}%
\psfrag{s19}[l][l]{\color[rgb]{0,0,0}residuals}%
\psfrag{s20}[l][l]{\color[rgb]{0,0,0}change relative to mean radius}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{}%
\psfrag{x08}[t][t]{}%
\psfrag{x09}[t][t]{}%
\psfrag{x10}[t][t]{}%
\psfrag{x11}[t][t]{}%
\psfrag{x12}[t][t]{}%
%
% yticklabels:
\psfrag{v01}[l][l]{0}%
\psfrag{v02}[l][l]{10}%
\psfrag{v03}[l][l]{20}%
\psfrag{v04}[l][l]{30}%
\psfrag{v05}[l][l]{40}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{2}%
\psfrag{v08}[r][r]{4}%
\psfrag{v09}[r][r]{6}%
\psfrag{v10}[r][r]{8}%
\psfrag{ypower3}[Bl][Bl]{}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{figure_3.eps}}%
\end{psfrags}%
%
% End figure_3.tex


==> images/flow-1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:20:12
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
\psfrag{v10}[r][r]{700}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{flow.eps}}%
\end{psfrags}%
%
% End pres.tex


==> images/flow.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:20:12
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
\psfrag{v10}[r][r]{700}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{flow.eps}}%
\end{psfrags}%
%
% End pres.tex


==> images/flow_close.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow_close}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 21:00:33
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
\psfrag{s08}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
\psfrag{v10}[r][r]{700}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{flow_close.eps}}%
\end{psfrags}%
%
% End flow_close.tex


==> images/flow_open.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow_open}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 20:57:35
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
\psfrag{s08}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
\psfrag{v10}[r][r]{700}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{flow_open.eps}}%
\end{psfrags}%
%
% End flow_open.tex


==> images/flow_open_close_asym.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{flow_open_close_asym}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           27-Apr-2014 18:47:15
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Flow Rate (ml/s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-200}%
\psfrag{v02}[r][r]{-100}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{100}%
\psfrag{v05}[r][r]{200}%
\psfrag{v06}[r][r]{300}%
\psfrag{v07}[r][r]{400}%
\psfrag{v08}[r][r]{500}%
\psfrag{v09}[r][r]{600}%
\psfrag{v10}[r][r]{700}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{flow_open_close_asym.eps}}%
\end{psfrags}%
%
% End flow_open_close_asym.tex


==> images/pres_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{pres_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           13-Oct-2013 10:24:34
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Time (s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Pressure (mmHg)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%\psfrag{s12}[l][l]{\color[rgb]{0,0,0}\huge Ventricular Pressure}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}\large Aortic Pressure}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}\large Ventricular Pressure}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{1.5}%
\psfrag{x05}[t][t]{2}%
\psfrag{x06}[t][t]{2.5}%
\psfrag{x07}[t][t]{3}%
\psfrag{x08}[t][t]{3.5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{40}%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{80}%
\psfrag{v06}[r][r]{100}%
\psfrag{v07}[r][r]{120}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{pres_2.eps}}%
\end{psfrags}%
%
% End pres_2.tex


==> images/pressure-1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{pressure}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:20:22
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Pressure (mmHg)\end{tabular}}%
\psfrag{s06}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Aorta N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Aorta N=256}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{40}%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{80}%
\psfrag{v06}[r][r]{100}%
\psfrag{v07}[r][r]{120}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{pressure.eps}}%
\end{psfrags}%
%
% End flow.tex


==> images/pressure.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{pressure}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-Jul-2014 14:20:22
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Pressure (mmHg)\end{tabular}}%
\psfrag{s06}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Aorta N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Aorta N=256}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Left Ventricle}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{40}%
\psfrag{v04}[r][r]{60}%
\psfrag{v05}[r][r]{80}%
\psfrag{v06}[r][r]{100}%
\psfrag{v07}[r][r]{120}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{pressure.eps}}%
\end{psfrags}%
%
% End flow.tex


==> images/residuals.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{residuals}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           13-Oct-2013 10:41:47
% eps bounding box:     15 cm x 11.25 cm
% comment:
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Residual (mm)\end{tabular}}%
\psfrag{s04}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Iteration Number\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{residuals.eps}}%
\end{psfrags}%
%
% End residuals.tex


==> images/sinus_asym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_asym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:40:59
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}Right}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}Left}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}Non-Coronary}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}Right}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.2}%
\psfrag{v02}[r][r]{-0.15}%
\psfrag{v03}[r][r]{-0.1}%
\psfrag{v04}[r][r]{-0.05}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.05}%
\psfrag{v07}[r][r]{0.1}%
\psfrag{v08}[r][r]{0.15}%
\psfrag{v09}[r][r]{0.2}%
\psfrag{v10}[r][r]{0.25}%
\psfrag{v11}[r][r]{0.3}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{sinus_asym_dx.eps}}%
\end{psfrags}%
%
% End sinus_asym_dx.tex


==> images/sinus_asym_dx_2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_asym_dx_2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Jul-2010 09:28:11
% eps bounding box:     15 cm x 11.2232 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.05}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.05}%
\psfrag{v04}[r][r]{0.1}%
\psfrag{v05}[r][r]{0.15}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.25}%
\psfrag{v08}[r][r]{0.3}%
\psfrag{v09}[r][r]{0.35}%
\psfrag{v10}[r][r]{0.4}%
\psfrag{v11}[r][r]{0.45}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{sinus_asym_dx_2.eps}}%
\end{psfrags}%
%
% End sinus_asym_dx_2.tex


==> images/sinus_closed.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_closed}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 09:16:52
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Time (s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Displacement (mm)\end{tabular}}%
\psfrag{s07}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}\Large N = 256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}\Large N = 128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}\Large N = 256}%
%
% xticklabels:
\psfrag{x01}[t][t]{\Large 1}%
\psfrag{x02}[t][t]{ }%
\psfrag{x03}[t][t]{\Large 2}%
\psfrag{x04}[t][t]{ }%
\psfrag{x05}[t][t]{\Large 3}%
\psfrag{x06}[t][t]{ }%
\psfrag{x07}[t][t]{\Large 4}%
%
% yticklabels:
\psfrag{v01}[r][r]{\Large 0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{\Large 0.2}%
\psfrag{v04}[r][r]{ }%
\psfrag{v05}[r][r]{\Large 0.4}%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{\Large 0.6}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{sinus_closed.eps}}%
\end{psfrags}%
%
% End sinus_closed.tex


==> images/sinus_open.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_open}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           21-Apr-2014 09:15:52
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Time (s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large Displacement (cm)\end{tabular}}%
\psfrag{s07}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}\Large N = 256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}\Large N = 128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}\Large N = 256}%
%
% xticklabels:
\psfrag{x01}[t][t]{\Large 1}%
\psfrag{x02}[t][t]{ }%
\psfrag{x03}[t][t]{\Large 2}%
\psfrag{x04}[t][t]{ }%
\psfrag{x05}[t][t]{\Large 3}%
\psfrag{x06}[t][t]{ }%
\psfrag{x07}[t][t]{\Large 4}%
%
% yticklabels:
\psfrag{v01}[r][r]{\Large 0}%
\psfrag{v02}[r][r]{ }%
\psfrag{v03}[r][r]{\Large 0.02}%
\psfrag{v04}[r][r]{ }%
\psfrag{v05}[r][r]{\Large 0.04}%
\psfrag{v06}[r][r]{ }%
\psfrag{v07}[r][r]{\Large 0.06}%
%
% Figure:
\resizebox{6cm}{!}{\includegraphics{sinus_open.eps}}%
\end{psfrags}%
%
% End sinus_open.tex


==> images/sinus_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 06:52:20
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Max Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}R}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}L}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N-C}%
\psfrag{s15}[l][l]{\color[rgb]{0,0,0}R}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{15}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{25}%
\psfrag{v04}[r][r]{30}%
\psfrag{v05}[r][r]{35}%
\psfrag{v06}[r][r]{40}%
\psfrag{v07}[r][r]{45}%
\psfrag{v08}[r][r]{50}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{sinus_sp1.eps}}%
\end{psfrags}%
%
% End sinus_sp1.tex


==> images/sinus_sym_dx.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_sym_dx}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:31:41
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Displacement (mm)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.05}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.05}%
\psfrag{v04}[r][r]{0.1}%
\psfrag{v05}[r][r]{0.15}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.25}%
\psfrag{v08}[r][r]{0.3}%
\psfrag{v09}[r][r]{0.35}%
\psfrag{v10}[r][r]{0.4}%
\psfrag{v11}[r][r]{0.45}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{sinus_sym_dx.eps}}%
\end{psfrags}%
%
% End sinus_sym_dx.tex


==> images/sinus_sym_sp1.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{sinus_sym_sp1}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           25-Apr-2014 07:08:22
% eps bounding box:     15 cm x 11.25 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time(s)\end{tabular}}%
\psfrag{s06}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}First Principal Stress (kPa)\end{tabular}}%
\psfrag{s10}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}N=256}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}N=128}%
\psfrag{s14}[l][l]{\color[rgb]{0,0,0}N=256}%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{1.5}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{2.5}%
\psfrag{x05}[t][t]{3}%
\psfrag{x06}[t][t]{3.5}%
\psfrag{x07}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{18}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{22}%
\psfrag{v04}[r][r]{24}%
\psfrag{v05}[r][r]{26}%
\psfrag{v06}[r][r]{28}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{32}%
\psfrag{v09}[r][r]{34}%
%
% Figure:
\resizebox{1\textwidth}{!}{\includegraphics{sinus_sym_sp1.eps}}%
\end{psfrags}%
%
% End sinus_sym_sp1.tex

